Enabling On-Device Large Language Model Personalization with Self-Supervised Data Selection and Synthesis

After a large language model (LLM) is deployed on edge devices, it is desirable for these devices to learn from user-generated conversation data to generate user-specific and personalized responses in real-time. However, user-generated data usually contains sensitive and private information, and uploading such data to the cloud for annotation is not preferred if not prohibited. While it is possible to obtain annotation locally by directly asking users to provide preferred responses, such annotations have to be sparse to not affect user experience. In addition, the storage of edge devices is usually too limited to enable large-scale fine-tuning with full user-generated data. It remains an open question how to enable on-device LLM personalization, considering sparse annotation and limited on-device storage. In this paper, we propose a novel framework to select and store the most representative data online in a self-supervised way. Such data has a small memory footprint and allows infrequent requests of user annotations for further fine-tuning. To enhance fine-tuning quality, multiple semantically similar pairs of question texts and expected responses are generated using the LLM. Our experiments show that the proposed framework achieves the best user-specific content-generating capability (accuracy) and fine-tuning speed (performance) compared with vanilla baselines. To the best of our knowledge, this is the very first on-device LLM personalization framework.

==> 3_proposed_original.tex <==
% \section{Proposed work}



% This paper proposes a framework on efficiently learn text data representations from semantic domain unlabeled user-generated input stream on-the-fly without accumulating a large dataset due to storage limitations on edge devices. To maintain the most representative data in the buffer such that learning from these data will benefit the model most, we propose a data refinement policy based on \textit{EDI Evaluator} by measuring the amount of information containing in each data and the quality of each data within each domain. Data containing high information and with high representative capability for each domain can effectively reflect the user personalized preference in certain domain and will be maintained in the buffer for further learning, while data with low information and less related to and representative in any domains will be dropped.

% \subsection{Framework Overview}
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\columnwidth]{fig_overview.png}
%   \caption{Overview of the framework. Fine-tune LLMs using data from data selection and following data generating.}
%   \label{fig:overview}
% \end{figure}

% As shown in Figure ~\ref{fig:overview}, the proposed framework has two stages. The first stage selects data which can most represent the user personalized preference. The second stage diversifies the selected data by generating semantically similar prompts towards each feedback in selected data.

% \subsection{Data Selection By EDI Evaluator}

% EDI evaluator, named by the three metrics explained later: \textbf{E}OE, \textbf{D}SS, and \textbf{I}DD, is designed to evaluate a small set of data. It estimates each input data based on the data itself and the comparative value of this data regarding the maintained data in buffers. In other words, the EDI evaluator will consistently interact with data buffers and dynamically update the data buffers. It contains three designed metrics to gradually decrease the amount of data required to compute and compare.

% % Data selector consists of two components: (1) three-step evaluator and (2) $To\_Train$ data holder. Data selector interacts with micro-controller (section 3.3). In general, data selector is designed to evaluate the informativity and importance of the user-generated data based on the past data in given certain hardware memory constraint. $To\_Train$ data holder functions as a buffer to temporarily save the informative and important user-generated texts.

% % \subsubsection{Three-step evaluator:}
% % There are three evaluation metrics in the three-step evaluator as it states. Each metric is used to filter out less informative text. The later metrics only consider the text with the higher value of the former metrics.


% \textit{\textbf{A. Entropy of Embedding (EOE)}}: User-generated texts can contain different amount of information. Given limited hardware resource, it is important to only keep the texts with high conciseness and information. Traditionally, the volume of information can be measured by calculating the entropy. However, such calculations can conduct high values given extremely short texts. To solve that, we apply logarithmic normalization into entropy calculation. Prior to calculate EOE, we tokenize the given text via a pretrained transformer language model tokenizer into numeric values. 

% Given the text $T$, its corresponding embedding $E(T)$, its text length $Len(T)$, the entropy of embedding (EOE) can be calculated as: 

% % Sentences can contain different amounts of information. A sentence with one to two modal particles represents less information than a sentence with rich vocabularies and complicated semantic expressions. Enlightened by in-context learning (ICL) \cite{han2023understanding}, we utilize entropy to quantify the information richness of each single user-generated text. To do this, the text will be tokenized and passed into a pretrained transformer language model to obtain the numeric embedding with semantic representations. Let \( T \) be a given text and its corresponding embedding be denoted as \( E(T) \). The entropy of the text \( T \), represented as \( EOE(T) \), is then calculated by:
% \begin{equation}
%     EOE(T) = \frac{-\sum_{e_i \in E(T)} p(e_i) \log p(e_i)}{\log(Len(T))}
% \end{equation}

% where \( E(T) = [e_1, e_2, ..., e_n] \) consists of components \( e_i \), and \( p(e_i) \) represents the probability distribution of these values, which can be estimated by discretizing the embedding values.
% % \item \textit{\textbf{Domain\&Semantic Score (DSS)}}: While EOE uses pretrained transformer language models to get the semantic embedding of the given text, the traditional embedding methods using GloVe or domain-specific such as medical are also important when evaluate and analyze the text. Within the texts with high EOE, we evaluate the text using a combination of multiple well-designed lexicon dictionaries. 
% % Let $T$ be a given text, $l_i$ belongs to a collection of lexicons clouding medical lexicon, emotion lexicon, GloVe embedding, etc. DSS can be calculated by the mean of ratios of all lexicons. (how much percent of tokens in T can be find in each lexcion dictionary)

% \textit{\textbf{B. Domain\&Semantic Score (DSS)}}: While EOE uses pretrained transformer language models to get the semantic embedding of the given text, the traditional embedding methods using GloVe or domain-specific such as medical are also important when evaluate and analyze the text. Each embedding method can be understood as domain. Within the texts with high EOE, we evaluate the text using a combination of multiple well-designed lexicon dictionaries. Let $T$ be the tokenized representation of the given text with \( |T| \) tokens, and let \(\mathcal{L} = \{l_1, l_2, \ldots, l_n\}\) be the collection of lexicons which includes the medical lexicon, emotion lexicon, GloVe embedding, etc. The DDS can be calculated as: 
% \begin{equation}
%     \text{DSS}(T) = \frac{1}{n} \sum_{i=1}^{n} \frac{|T_{l_i}|}{|T|}
% \end{equation}
% For each lexicon \( l_i \), let \( T_{l_i} \) be the subset of tokens from \( T \) that can be found in \( l_i \). The ratio \( R(l_i) \) of tokens in \( T \) found in lexicon \( l_i \) is then given by \( \frac{|T_{l_i}|}{|T|} \).

% \textit{\textbf{C. In-Domain Distinction (IDD)}}: With high EOE text selected, we further evaluate the semantic quality of these text. While DSS leverages all lexicon dictionaries, it diminishes the significance of the dominant domain, in which the $R(l_i)$ for given text $T$ is higher than all others. We tag each text with the dominant domain, and grouping texts based on their dominant domain tags.

% Within each group, the certain amount of texts with the highest DSS will be maintained by micro-controller (section 3.3) to form a high-quality group, and the texts with the same tag and relative high DSS will be temporarily held by micro-controller until reaching certain amount. Then a text with the most dissimilarity  from these temproarily held texts will be added by micro-controller into the high-quality group. 

% % Each each temporary text $T_{temp}$ will compare with each high-quality text $T_{hq}$ via cosine similarity, and get the average value. The $T_{temp}$ with the highest average value will be picked.
% Given a text \( T \), we define its dominant domain \( l_{dom}(T) \) by its highest lexical overlap:
% \begin{equation}
% \label{equ:dominant_domain}
%     l_{dom}(T) = \arg \max_{l_i \in \mathcal{L}} R(l_i)
% \end{equation}

% % Given a collection of texts, we group them by their dominant domain into a set of groups \( \mathcal{G} = \{ G_1, G_2, \ldots, G_m \} \). For each group \( G_j \), we define \( T_{hq} \) as the high-quality texts. For each \( T_{temp} \) in \( G_j \):
% % \begin{equation}
% %     \text{AvgSim}(T_{temp}, T_{hq}) = \frac{1}{|T_{hq}|} \sum_{t \in T_{hq}} \frac{T_{temp} \cdot t}{\|T_{temp}\| \|t\|}
% % \end{equation}

% Given a collection of texts, we group them by their dominant domain into a set of groups \( \mathcal{G} = \{ G_1, G_2, \ldots, G_m \} \). For each group \( G_j \), we define \( T_{hq} \) as the high-quality texts. For each \( T_{temp} \) in \( G_j \), let \( \mathbf{E}_{temp} \) and \( \mathbf{E}_t \) represent the semantic embeddings of \( T_{temp} \) and text \( t \) in \( T_{hq} \) respectively, obtained using a pretrained transformer model. Then the average similarity is computed as:

% \begin{equation}
%     \text{AvgSim}(T_{temp}, T_{hq}) = \frac{1}{|T_{hq}|} \sum_{t \in T_{hq}} \frac{\mathbf{E}_{temp} \cdot \mathbf{E}_t}{\| \mathbf{E}_{temp} \|_2 \cdot \| \mathbf{E}_t \|_2}
% \end{equation}


% From which, the text to be added to the high-quality group is:
% \begin{equation}
%     T_{temp^*} = \arg \max_{T_{temp}} \text{AvgSim}(T_{temp}, T_{hq})
% \end{equation}

% % \subsubsection{$To\_Train$ data holder:} The text data after three-step evaluator will be held in $To\_Train$ data holder with the guiding of micro-controller. Micro-controller decides what data should be kept and what data should be updated in terms of hardware efficiency. When the capacity of the data holder is approaching to the limit, the data selector sends out the data. 

% \subsection{Domain Buffers}

% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\columnwidth]{fig_mc_data_selector.png}
%   % \caption{Micro-Controller guides data selector and uses the three-step evaluator to update the data loader in data selector. }
%   \caption{Domain Buffers. The EDI evaluator works with domain buffers to efficiently select data}
%   \label{fig:mc_data_selector}
% \end{figure}

% Domain buffers maintain the selected data based on EDI evaluator and forward the selected data to format the synthetic data which is used to LLM fine-tuning, as shown in Figure ~\ref{fig:overview}. We propose domain buffers to mange and process user input data with spatial and computational benefit.

% % When the input data has low frequent need to compare with the data in the buffer, a simple data buffer is sufficient. In our work, the calculation of EDI evaluator replies on the data maintained in the buffer. As shown in Figure. ~\ref{fig:overview}, we design a different data buffer paradigm called domain buffers to solve two problems: (1) Due to the high frequent buffer-maintained data access and retrieve need, and each time we need to select data with specific domain to complete the EDI evaluation, it is computationally inefficient to maintain selected data in a single data buffer. (2) The "cold start" problem widely exists in small-scale data learning tasks, not to mention the buffer will be regularly cleaned due to the limited storage. Without enough amount of existing data, calculating of the EDI evaluator is less effective since the poor initial selected data can lead to ineffective following in-domain distinct data selection.

% % \begin{algorithm}
% % \caption{On-Device LLM(input)}
% % \begin{algorithmic}
% % \STATE //Domain\_Buffers is a global variable
% % \STATE $EOE \gets \text{calculate\_EOE}(input)$
% % \STATE $domain \gets \text{get\_domain}(input)$
% % \STATE $DSS \gets \text{calculate\_DSS}(input)$
% % \STATE $buffer \gets \text{Domain\_Buffers}[domain]$
% % \STATE $selected\_data \gets \text{None}$
% % \IF{not $buffer.primary.full$}
% %     \IF{not $buffer.cache.full$}
% %         \STATE $buffer.primary.append((input, EOE, DSS))$
% %     \ELSE
% %         \STATE $buffer.primary.append(\text{buffer.cache.high\_EOE\_DSS})$
% %         \STATE $buffer.cache.clean()$
% %     \ENDIF
% % \ELSE
% %     \IF{not $buffer.secondary.full$ \AND $buffer.cache.full$}
% %         \STATE $buffer.secondary.append(\text{high\_IDD}(buffer.cache))$
% %         \STATE $buffer.cache.clean()$
% %     \ENDIF
% %     \IF{$buffer.secondary.full$}
% %         \STATE $selected\_data \gets buffer.primary + buffer.secondary$
% %     \ENDIF
% % \ENDIF
% % \IF{$selected\_data$}
% %     \STATE $\text{finetune\_LLM}(selected\_data)$
% % \ENDIF
% % \end{algorithmic}
% % \end{algorithm}

% % Environment to change margins
% \newenvironment{changemargin}[2]{%
%     \begin{list}{}{%
%         \setlength{\topsep}{0pt}%
%         \setlength{\leftmargin}{#1}%
%         \setlength{\rightmargin}{#2}%
%         \setlength{\parsep}{0pt}%
%         \setlength{\partopsep}{0pt}%
%     }%
%     \item[]}{\end{list}}
% \begin{algorithm}
% \caption{Domain\_Buffers logic}
% \label{alg:on-device_llm}
% \begin{changemargin}{1em}{0em}

% // Buffers is a global variable to hold data for all domains\\
% % EOE, DSS = calculate\_EOE(input), calculate\_DSS(input)   \\
% % domain, buffer = get\_domain(input), Domain\_Buffers[domain] \\
% % % buffer = Domain\_Buffers[domain] \\
% % selected\_data = None

% \textbf{if} buffer.primary not full \\
% \begin{changemargin}{1em}{0em}
%     \textbf{if} buffer.cache not full\textbf{:} buffer.cache.append(input: (EOE, DSS))  \\
%     % \begin{changemargin}{1em}{0em}
%     %     buffer.cache.append(input: (EOE, DSS)) \\
%     % \end{changemargin}
%     \textbf{elif} buffer.primary.min > buffer.cache.high\_EOE\_DSS \\
%     \begin{changemargin}{1em}{0em}
%         buffer.primary.append(buffer.cache.high\_EOE\_DSS) \\
%         % buffer.cache.clean() \\
%     \end{changemargin}
%     \textbf{else:} replace buffer.primary.min\\
%     % \begin{changemargin}{1em}{0em}
%     %     buffer.primary.append(buffer.cache.high\_EOE\_DSS) \\
%     %     % buffer.cache.clean() \\
%     % \end{changemargin}
% \end{changemargin}
% \textbf{else} \\
% \begin{changemargin}{1em}{0em}
%     \textbf{if} buffer.secondary not full and buffer.cache full \\
%     \begin{changemargin}{1em}{0em}
%         buffer.secondary.append(high\_IDD(buffer.cache)) \\
%         % buffer.cache.clean() \\
%     \end{changemargin}
%     \textbf{if} buffer.secondary full \\
%     \begin{changemargin}{1em}{0em}
%         selected\_data = buffer.primary + buffer.secondary \\
%         finetune\_LLM(selected\_data) \\
%     \end{changemargin}
% \end{changemargin}
% \textbf{if} buffer.cache full: buffer.cache.clean()
% % \textbf{if} selected\_data \\
% % \begin{changemargin}{1em}{0em}
% %     finetune\_LLM(selected\_data) \\
% % \end{changemargin}
% \end{changemargin}
% \end{algorithm}

% % As shown in Figure ~\ref{fig:mc_data_selector}, each domain is assigned an individual buffer which contains three sectors. The same type of sectors in all buffers have equal capacity. Every input data will be placed in cache sector first in the buffer belongs to its domain. When the cache sector is full, the input with high EOE and DSS will fill the primary sector first. When the primary sector is full, the secondary sector will be filled by the input from full cache sector with high IDD. The number of inputs with high EOE and DSS or with high IDD can be changed to alter the data accumulation speed. The cache sector will be emptied once its data fill primary or secondary sector. 
% As shown in Figure ~\ref{fig:mc_data_selector}, each domain is assigned an individual buffer, which contains three sectors. The same type of sectors in all buffers have equal capacity. Every input data will be placed in the cache sector first in the buffer belonging to its domain. When the cache sector is full, the input with high EOE and DSS will fill the primary sector first. When the primary sector is full, the secondary sector will be filled by the input from the full cache sector with high IDD. The number of inputs with high EOE and DSS or with high IDD can be changed to alter the data accumulation speed. We use \textbf{selection rate} to represent the ratio of high-ranked text to be selected in cache sector. The cache sector will be emptied once its data fills the primary or secondary sector. 



% % When the secondary sector in any buffers is full, the data in primary sector and secondary sector in every buffer will be extracted and used to fine-tune the LLM. We design \textbf{early stop} strategy to avoid the potential data wasting when the user-generated data concentrating on certain domains. And the personalized LLM can be fine-tuned will less data and learn user-specific data faster.
% When the secondary sector in any buffer is full, the data in the primary and secondary sectors of every buffer will be extracted and used to fine-tune the LLM. We designed an \textbf{early stop} strategy to avoid potential data waste when the user-generated data concentrates on certain domains. Thus, the personalized LLM can be fine-tuned with less data and learn user-specific data faster.

% % As shown in Algorithm ~\ref{alg:on-device_llm}, this logic enables evaluate user input in stream data in a small scale and save storage and computational cost compared with selecting data from a large scale data. 
% As shown in Algorithm ~\ref{alg:on-device_llm}, this logic enables the evaluation of user input in streaming data on a small scale and saves storage and computational costs compared with selecting data on a large scale.


% \subsection{Efficiency of Data Selection}

% Data selection is a process where domain buffers fill the primary and secondary sectors using EDI evaluator. To analyze the efficiency of data selection, we can split the data selection into three parts: (1) complexity of EDI calculation, (2) complexity of retrieval data with high EOE and DSS, and (3) complexity of retrieval data with high IDD. 

% % The proposed EDI evaluator collaborating with domain buffers can effectively select data in terms of spatial and computational efficiency. To analyze the data selection efficiency, 
% \subsubsection{Complexity of EDI Calculation}
% The computational complexity of the EDI calculation involves the tokenization of text, calculation of embedding entropy (EOE), and the domain and semantic score (DSS). Let $N$ be the number of texts, $M$ the average number of tokens per text, and $V$ the size of the vocabulary used in tokenization and embedding.

% \begin{itemize}
%     \item \textbf{Tokenization:} The complexity of tokenizing a text using a pretrained transformer language model tokenizer is $O(M)$.
%     \item \textbf{Entropy of Embedding (EOE):} To compute EOE, we calculate the entropy for each embedding vector. The complexity of this step is $O(M \cdot d)$, where $d$ is the dimensionality of the embeddings.
%     \item \textbf{Domain \& Semantic Score (DSS):} DSS computation involves comparing tokenized text against multiple lexicon dictionaries, resulting in a complexity of $O(M \cdot L)$, where $L$ is the number of lexicons.
% \end{itemize}

% Therefore, the overall complexity for the EDI calculation is $O(N \cdot (M + M \cdot d + M \cdot L)) = O(N \cdot M \cdot (1 + d + L))$.

% \subsubsection{Complexity of Retrieval with High EOE and DSS}
% To retrieve data with high EOE and DSS, we sort texts based on their scores. Assuming the use of an efficient sorting algorithm like heapsort or mergesort:

% \begin{itemize}
%     \item The complexity is $O(N \cdot \log N)$ for sorting based on EOE and DSS scores.
% \end{itemize}

% \subsubsection{Complexity of Retrieval with High IDD}
% The retrieval of data with high IDD involves grouping by dominant domain and then selecting the most distinctive texts within each group:

% \begin{itemize}
%     \item \textbf{Grouping:} The complexity of grouping texts by their dominant domain is $O(N)$.
%     \item \textbf{Selection:} For each domain, selecting the text with the maximum average similarity involves a pairwise comparison within the group. If $g$ is the average group size, the complexity is $O(g^2)$ for each group.
% \end{itemize}

% Given that there are $D$ domains, the total complexity for retrieval with high IDD is $O(N + D \cdot g^2)$.

% Combining these complexities gives us an overall picture of the computational effort required for data selection within the EDI evaluator framework.

% % \subsubsection{Baseline Method Complexity}
% % In the baseline method, where we do not utilize primary and secondary sectors and instead store all data in a single buffer, the computational complexity significantly increases due to the pairwise distinctness computations required for every two pieces of data.

% % Assuming we have $N$ data points and we need to calculate the distinctness between every pair:

% % \begin{itemize}
% %     \item The complexity for computing distinctness between two data points is $O(1)$.
% %     \item To compute the distinctness across all pairs, we perform this computation for each pair, resulting in a complexity of $O(N^2)$, since there are $\frac{N \cdot (N - 1)}{2}$ pairs.
% % \end{itemize}

% % \textit{\textbf{Domain Buffer}}:
% \subsection{Enhance Selected Data by Data Synthesis}

% To effectively fine-tune LLM, semantically similar prompts can increase the model confidence in generating certain expected answers. From this perspective, the large-scaled dataset is necessary due to the high probability to contain such data. However, with significantly limited data, the learning is insufficient for the model to generate certain expected text. To minimize the insufficiency, we propose data synthesis, in which the prompts in selected data are used to generate more similar prompts within a computational acceptable range.

% When the data buffer is full and output the selected data, the deployed LLM, as a generative language model, can be reused as a data generator to diversify the selected prompts. With considering the storage and computational resource constraint, the data synthesis only linearly increase the data size. 


% % \begin{algorithm}
% % \caption{On-Device LLM(input)}
% % \begin{algorithmic}
% % % \STATE Initialize \textbf{Buffers} with domain and data list
% % % \REQUIRE $\textbf{Buffers} \gets \{ 'domain' : \text{data list} \}$
% % % \FUNCTION{onDeviceLLM}{$input$}
% % \STATE { //Domain\_Buffers is a global variable}
% % \STATE $EOE \gets CalculateEOE(input)$
% % \STATE $domain \gets GetDomain(input)$
% % \STATE $DSS \gets CalculateDSS(input)$
% % \STATE $buffer \gets \textbf{Buffers}[domain]$
% % \IF{space in $buffer.primary$}
% %     \STATE $buffer.primary.append((input, EOE, DSS))$
% % \ELSIF{space in $buffer.cache$}
% %     \STATE $buffer.cache.append((input, EOE, DSS))$
% %     \STATE $buffer.primary.append(High\_EOE\_DSS(buffer.cache))$
% %     \STATE $buffer.cache.clear()$
% % \ELSIF{space in $buffer.secondary$}
% %     \STATE $buffer.secondary.append(High\_IDD(buffer.cache))$
% %     \STATE $buffer.cache.clear()$
% % \ENDIF
% % \STATE $SelectedData \gets buffer.primary + buffer.secondary$
% % \IF{$SelectedData$ is not empty}
% %     \STATE $FinetuneLLM(SelectedData)$
% % \ENDIF
% % \end{algorithmic}
% % \end{algorithm}



% % Micro-controller work with IDD.

% % We enable the micro-controller to decide the volume of each dominant domain group. In each group, certain amount of text with the highest DSS will be filled until reach a primary threshold. Then the micro-controller will assign an temporary buffer to each group to hold certain amount of text with high but not higher DDS than the text within the primary threshold. Once the volume of the temporary buffer reach a threshold (secondary threshold), the text with the most dissimilarity compare with the texts within primary threshold will be selected. 
% \subsection{LLM Personalization Metric}

% % Evaluate how much the generated text containing relates to the user-specific information is important to LLM for on-device learning. The user-specific information contains the user-LLM interaction history, which can be safely retained in private devices. However, a widely used personalization metric for language model is lacking since it is difficult to contain the conceptual range of personalized information which also leads to the difficulty of quantifying the metric.
% Our framework aims to enhance the LLM capability of causal inference regarding specific users. Different simpler tasks like sequence classification, causal inference cannot be evaluated by prediction accuracy. However, assessing the relevance of generated text to user-specific information is pivotal for on-device learning in LLMs. Such user-specific information encompasses the history of interactions between the user and the LLM, which can be securely stored on private devices. Nonetheless, there is an absence of a universally-accepted personalization metric for language models. This is mainly due to the challenges in capturing the broad spectrum of personalized information, which subsequently makes the metric difficult to quantify.

% % As an alternative, we can measure the generative language model personalization performance via their generated content regarding same prompts. This idea is same as the daily human interaction, where the past and verified answer should be made when people receive the same questions. To quantify the amount of past information the language model can generate, we propose to calculate the cosine similarity of the semantic embedding of the generated content and the original human answers.
% As a solution, we propose assessing the personalization performance of generative language models based on the content they produce in response to identical prompts. This approach mirrors everyday human interactions, wherein individuals are expected to provide consistent and validated answers when posed with the same questions. To quantify the model's ability to reproduce past information, we suggest calculating the cosine similarity between the semantic embeddings of the generated content and the original human responses.

% Given two texts: the original text \( T_o \) and the generated text \( T_g \), we introduce the \textbf{Personalized Correlated Score (PCS)} as:
% \begin{equation}
%     \text{PCS}(T_o, T_g) = \frac{\mathbf{E}_o \cdot \mathbf{E}_g}{\| \mathbf{E}_o \|_2 \cdot \| \mathbf{E}_g \|_2}
% \end{equation}
% % \text{PCS}(T_o, T_g) = \frac{\mathbf{E}_o \cdot \mathbf{E}_g}{\| \mathbf{E}_o \|_2 \cdot \| \mathbf{E}_g \|_2},
% % \]
% where $\mathbf{E}_o$ and $\mathbf{E}_g$ represent the semantic embeddings of \( T_o \) and \( T_g \) respectively, obtained using a pretrained transformer model.


==> 3_proposed_v1.tex <==
% \section{Proposed work}

% % This paper proposes a framework to efficiently learn user-generated data from unprocessed and unlabeled input stream on edge devices. The designed domain buffers collaborating with EDI evaluator, which will be elaborated in the following, can efficiently maintain the data mostly related to users and represent the user-specific information. The small size selected data, after data synthesis to augment the data, will be used to fine-tune LLM. 
% This paper introduces a framework that learns from user-generated content directly from unprocessed, unlabeled data streams on edge devices. The framework utilizes designed domain buffers in conjunction with an EDI evaluator—details of which are forthcoming—that effectively preserve the most user-relevant data, capturing information unique to each user. The selected data, once expanded through data synthesis, is employed to fine-tune large language models (LLMs).

% % This paper proposes a framework on efficiently learn text data representations from semantic domain unlabeled user-generated input stream on-the-fly without accumulating a large dataset due to storage limitations on edge devices. To maintain the most representative data in the buffer such that learning from these data will benefit the model most, we propose a data refinement policy based on \textit{EDI Evaluator} by measuring the amount of information containing in each data and the quality of each data within each domain. Data containing high information and with high representative capability for each domain can effectively reflect the user personalized preference in certain domain and will be maintained in the buffer for further learning, while data with low information and less related to and representative in any domains will be dropped.

% In this section, we will first present the framework overview in section 3.1. Then we will introduce EDI evaluator in section 3.2 and domain buffers in section 3.3, both together work for data selection. After that, we evaluate the efficiency in section 3.4 for the data selection we introduced. Later on, we explain data synthesis in section 3.5 which is used to the selected data. Finally, we introduce a new metric in section 3.6 to evaluate the personalized LLM fine-tuning effect.

% \subsection{Framework Overview}
% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\columnwidth]{fig_overview.png}
%   \caption{Overview of the framework. Fine-tune LLMs using data from data selection and following data generating.}
%   \label{fig:overview}
% \end{figure}

% As shown in Figure ~\ref{fig:overview}, the proposed framework contains three components: EDI evaluator, domain buffers, and data synthesis. EDI evaluator collaborating with domain buffers to select highly user-related data, which will be sent to data synthesis to augment and format the final data for LLM to fine-tune. In EDI evaluator, the input data will be calculated based on different metrics and saved in domain buffers. Domain buffers consist of many data buffers, where each buffer only hold data belongs to the same domain. Data synthesis as shwon in Figure ~\ref{fig:overview}, augments selected data by diverse the prompt.

% % As shown in Figure ~\ref{fig:overview}, the proposed framework has two stages. The first stage selects data which can most represent the user personalized preference. The second stage diversifies the selected data by generating semantically similar prompts towards each feedback in selected data.

% \subsection{Data Selection By EDI Evaluator}

% EDI evaluator is designed to quantify the value of input data. It consists of three metrics including \textbf{E}OE, \textbf{D}SS, and \textbf{I}DD. The three metrics work with domain buffers to select data which are highly user-related. In this section, we explain how to calculate the three metrics and why they are used.

% % EDI evaluator, named by the three metrics explained later: \textbf{E}OE, \textbf{D}SS, and \textbf{I}DD, is designed to evaluate a small set of data. It estimates each input data based on the data itself and the comparative value of this data regarding the maintained data in buffers. In other words, the EDI evaluator will consistently interact with data buffers and dynamically update the data buffers. It contains three designed metrics to gradually decrease the amount of data required to compute and compare.

% % Data selector consists of two components: (1) three-step evaluator and (2) $To\_Train$ data holder. Data selector interacts with micro-controller (section 3.3). In general, data selector is designed to evaluate the informativity and importance of the user-generated data based on the past data in given certain hardware memory constraint. $To\_Train$ data holder functions as a buffer to temporarily save the informative and important user-generated texts.

% % \subsubsection{Three-step evaluator:}
% % There are three evaluation metrics in the three-step evaluator as it states. Each metric is used to filter out less informative text. The later metrics only consider the text with the higher value of the former metrics.


% \textit{\textbf{A. Entropy of Embedding (EOE)}}: User-generated texts can contain different amount of information. Given limited hardware resource, it is important to only keep the texts with high conciseness and information. Traditionally, the volume of information can be measured by calculating the entropy. However, such calculations can conduct high values given extremely short texts. To solve that, we apply logarithmic normalization into entropy calculation. Prior to calculate EOE, we tokenize the given text via a pretrained transformer language model tokenizer into numeric values. 

% Given the text $T$, its corresponding embedding $E(T)$, its text length $Len(T)$, the entropy of embedding (EOE) can be calculated as: 

% % Sentences can contain different amounts of information. A sentence with one to two modal particles represents less information than a sentence with rich vocabularies and complicated semantic expressions. Enlightened by in-context learning (ICL) \cite{han2023understanding}, we utilize entropy to quantify the information richness of each single user-generated text. To do this, the text will be tokenized and passed into a pretrained transformer language model to obtain the numeric embedding with semantic representations. Let \( T \) be a given text and its corresponding embedding be denoted as \( E(T) \). The entropy of the text \( T \), represented as \( EOE(T) \), is then calculated by:
% \begin{equation}
%     EOE(T) = \frac{-\sum_{e_i \in E(T)} p(e_i) \log p(e_i)}{\log(Len(T))}
% \end{equation}

% where \( E(T) = [e_1, e_2, ..., e_n] \) consists of components \( e_i \), and \( p(e_i) \) represents the probability distribution of these values, which can be estimated by discretizing the embedding values.
% % \item \textit{\textbf{Domain\&Semantic Score (DSS)}}: While EOE uses pretrained transformer language models to get the semantic embedding of the given text, the traditional embedding methods using GloVe or domain-specific such as medical are also important when evaluate and analyze the text. Within the texts with high EOE, we evaluate the text using a combination of multiple well-designed lexicon dictionaries. 
% % Let $T$ be a given text, $l_i$ belongs to a collection of lexicons clouding medical lexicon, emotion lexicon, GloVe embedding, etc. DSS can be calculated by the mean of ratios of all lexicons. (how much percent of tokens in T can be find in each lexcion dictionary)

% \textit{\textbf{B. Domain\&Semantic Score (DSS)}}: While EOE uses pretrained transformer language models to get the semantic embedding of the given text, the traditional embedding methods using GloVe or domain-specific such as medical are also important when evaluate and analyze the text. Each embedding method can be understood as domain. Within the texts with high EOE, we evaluate the text using a combination of multiple well-designed lexicon dictionaries. Let $T$ be the tokenized representation of the given text with \( |T| \) tokens, and let \(\mathcal{L} = \{l_1, l_2, \ldots, l_n\}\) be the collection of lexicons which includes the medical lexicon, emotion lexicon, GloVe embedding, etc. The DDS can be calculated as: 
% \begin{equation}
%     \text{DSS}(T) = \frac{1}{n} \sum_{i=1}^{n} \frac{|T_{l_i}|}{|T|}
% \end{equation}
% For each lexicon \( l_i \), let \( T_{l_i} \) be the subset of tokens from \( T \) that can be found in \( l_i \). The ratio \( R(l_i) \) of tokens in \( T \) found in lexicon \( l_i \) is then given by \( \frac{|T_{l_i}|}{|T|} \).

% \textit{\textbf{C. In-Domain Distinction (IDD)}}: With high EOE text selected, we further evaluate the semantic quality of these text. While DSS leverages all lexicon dictionaries, it diminishes the significance of the dominant domain, in which the $R(l_i)$ for given text $T$ is higher than all others. We tag each text with the dominant domain, and grouping texts based on their dominant domain tags.

% Within each group, the certain amount of texts with the highest DSS will be maintained by micro-controller (section 3.3) to form a high-quality group, and the texts with the same tag and relative high DSS will be temporarily held by micro-controller until reaching certain amount. Then a text with the most dissimilarity  from these temproarily held texts will be added by micro-controller into the high-quality group. 

% % Each each temporary text $T_{temp}$ will compare with each high-quality text $T_{hq}$ via cosine similarity, and get the average value. The $T_{temp}$ with the highest average value will be picked.
% Given a text \( T \), we define its dominant domain \( l_{dom}(T) \) by its highest lexical overlap:
% \begin{equation}
% \label{equ:dominant_domain}
%     l_{dom}(T) = \arg \max_{l_i \in \mathcal{L}} R(l_i)
% \end{equation}

% % Given a collection of texts, we group them by their dominant domain into a set of groups \( \mathcal{G} = \{ G_1, G_2, \ldots, G_m \} \). For each group \( G_j \), we define \( T_{hq} \) as the high-quality texts. For each \( T_{temp} \) in \( G_j \):
% % \begin{equation}
% %     \text{AvgSim}(T_{temp}, T_{hq}) = \frac{1}{|T_{hq}|} \sum_{t \in T_{hq}} \frac{T_{temp} \cdot t}{\|T_{temp}\| \|t\|}
% % \end{equation}

% Given a collection of texts, we group them by their dominant domain into a set of groups \( \mathcal{G} = \{ G_1, G_2, \ldots, G_m \} \). For each group \( G_j \), we define \( T_{hq} \) as the high-quality texts. For each \( T_{temp} \) in \( G_j \), let \( \mathbf{E}_{temp} \) and \( \mathbf{E}_t \) represent the semantic embeddings of \( T_{temp} \) and text \( t \) in \( T_{hq} \) respectively, obtained using a pretrained transformer model. Then the average similarity is computed as:

% \begin{equation}
%     \text{AvgSim}(T_{temp}, T_{hq}) = \frac{1}{|T_{hq}|} \sum_{t \in T_{hq}} \frac{\mathbf{E}_{temp} \cdot \mathbf{E}_t}{\| \mathbf{E}_{temp} \|_2 \cdot \| \mathbf{E}_t \|_2}
% \end{equation}


% From which, the text to be added to the high-quality group is:
% \begin{equation}
%     T_{temp^*} = \arg \max_{T_{temp}} \text{AvgSim}(T_{temp}, T_{hq})
% \end{equation}

% % \subsubsection{$To\_Train$ data holder:} The text data after three-step evaluator will be held in $To\_Train$ data holder with the guiding of micro-controller. Micro-controller decides what data should be kept and what data should be updated in terms of hardware efficiency. When the capacity of the data holder is approaching to the limit, the data selector sends out the data. 

% \subsection{Domain Buffers}

% \begin{figure}[t!]
%   \centering
%   \includegraphics[width=\columnwidth]{fig_mc_data_selector.png}
%   % \caption{Micro-Controller guides data selector and uses the three-step evaluator to update the data loader in data selector. }
%   \caption{Domain Buffers. The EDI evaluator works with domain buffers to efficiently select data}
%   \label{fig:mc_data_selector}
% \end{figure}

% Domain buffers utilize EDI evaluator to formalize selected data. As its name states, domain buffers consist of many data buffers. We assign each domain an individual buffer to enable computationally efficient EDI calculation, which will be elaborated in section 3.4. In this section, we demonstrate the operating logic of domain buffers.

% % Domain buffers maintain the selected data based on EDI evaluator and forward the selected data to format the synthetic data which is used to LLM fine-tuning, as shown in Figure ~\ref{fig:overview}. We propose domain buffers to mange and process user input data with spatial and computational benefit.

% % When the input data has low frequent need to compare with the data in the buffer, a simple data buffer is sufficient. In our work, the calculation of EDI evaluator replies on the data maintained in the buffer. As shown in Figure. ~\ref{fig:overview}, we design a different data buffer paradigm called domain buffers to solve two problems: (1) Due to the high frequent buffer-maintained data access and retrieve need, and each time we need to select data with specific domain to complete the EDI evaluation, it is computationally inefficient to maintain selected data in a single data buffer. (2) The "cold start" problem widely exists in small-scale data learning tasks, not to mention the buffer will be regularly cleaned due to the limited storage. Without enough amount of existing data, calculating of the EDI evaluator is less effective since the poor initial selected data can lead to ineffective following in-domain distinct data selection.

% % \begin{algorithm}
% % \caption{On-Device LLM(input)}
% % \begin{algorithmic}
% % \STATE //Domain\_Buffers is a global variable
% % \STATE $EOE \gets \text{calculate\_EOE}(input)$
% % \STATE $domain \gets \text{get\_domain}(input)$
% % \STATE $DSS \gets \text{calculate\_DSS}(input)$
% % \STATE $buffer \gets \text{Domain\_Buffers}[domain]$
% % \STATE $selected\_data \gets \text{None}$
% % \IF{not $buffer.primary.full$}
% %     \IF{not $buffer.cache.full$}
% %         \STATE $buffer.primary.append((input, EOE, DSS))$
% %     \ELSE
% %         \STATE $buffer.primary.append(\text{buffer.cache.high\_EOE\_DSS})$
% %         \STATE $buffer.cache.clean()$
% %     \ENDIF
% % \ELSE
% %     \IF{not $buffer.secondary.full$ \AND $buffer.cache.full$}
% %         \STATE $buffer.secondary.append(\text{high\_IDD}(buffer.cache))$
% %         \STATE $buffer.cache.clean()$
% %     \ENDIF
% %     \IF{$buffer.secondary.full$}
% %         \STATE $selected\_data \gets buffer.primary + buffer.secondary$
% %     \ENDIF
% % \ENDIF
% % \IF{$selected\_data$}
% %     \STATE $\text{finetune\_LLM}(selected\_data)$
% % \ENDIF
% % \end{algorithmic}
% % \end{algorithm}

% % Environment to change margins
% \newenvironment{changemargin}[2]{%
%     \begin{list}{}{%
%         \setlength{\topsep}{0pt}%
%         \setlength{\leftmargin}{#1}%
%         \setlength{\rightmargin}{#2}%
%         \setlength{\parsep}{0pt}%
%         \setlength{\partopsep}{0pt}%
%     }%
%     \item[]}{\end{list}}
% \begin{algorithm}
% \caption{Domain\_Buffers logic}
% \label{alg:on-device_llm}
% \smaller
% \begin{changemargin}{1em}{0em}

% // Buffers is a global variable to hold data for all domains\\
% % EOE, DSS = calculate\_EOE(input), calculate\_DSS(input)   \\
% % domain, buffer = get\_domain(input), Domain\_Buffers[domain] \\
% % % buffer = Domain\_Buffers[domain] \\
% % selected\_data = None

% \textbf{if} buffer.primary not full \\
% \begin{changemargin}{1em}{0em}
%     \textbf{if} buffer.cache not full\textbf{:} buffer.cache.append(input: (EOE, DSS))  \\
%     % \begin{changemargin}{1em}{0em}
%     %     buffer.cache.append(input: (EOE, DSS)) \\
%     % \end{changemargin}
%     \textbf{elif} buffer.primary.min > buffer.cache.high\_EOE\_DSS \\
%     \begin{changemargin}{1em}{0em}
%         buffer.primary.append(buffer.cache.high\_EOE\_DSS) \\
%         % buffer.cache.clean() \\
%     \end{changemargin}
%     \textbf{else:} replace buffer.primary.min\\
%     % \begin{changemargin}{1em}{0em}
%     %     buffer.primary.append(buffer.cache.high\_EOE\_DSS) \\
%     %     % buffer.cache.clean() \\
%     % \end{changemargin}
% \end{changemargin}
% \textbf{else} \\
% \begin{changemargin}{1em}{0em}
%     \textbf{if} buffer.secondary not full and buffer.cache full \\
%     \begin{changemargin}{1em}{0em}
%         buffer.secondary.append(high\_IDD(buffer.cache)) \\
%         % buffer.cache.clean() \\
%     \end{changemargin}
%     \textbf{if} buffer.secondary full \\
%     \begin{changemargin}{1em}{0em}
%         selected\_data = buffer.primary + buffer.secondary \\
%         finetune\_LLM(selected\_data) \\
%     \end{changemargin}
% \end{changemargin}
% \textbf{if} buffer.cache full: buffer.cache.clean()
% % \textbf{if} selected\_data \\
% % \begin{changemargin}{1em}{0em}
% %     finetune\_LLM(selected\_data) \\
% % \end{changemargin}
% \end{changemargin}
% \end{algorithm}

% % As shown in Figure ~\ref{fig:mc_data_selector}, each domain is assigned an individual buffer which contains three sectors. The same type of sectors in all buffers have equal capacity. Every input data will be placed in cache sector first in the buffer belongs to its domain. When the cache sector is full, the input with high EOE and DSS will fill the primary sector first. When the primary sector is full, the secondary sector will be filled by the input from full cache sector with high IDD. The number of inputs with high EOE and DSS or with high IDD can be changed to alter the data accumulation speed. The cache sector will be emptied once its data fill primary or secondary sector. 
% As shown in Figure ~\ref{fig:mc_data_selector}, each domain is assigned an individual buffer, which contains three sectors. The same type of sectors in all buffers have equal capacity. Every input data will be placed in the cache sector first in the buffer belonging to its domain. When the cache sector is full, the input with high EOE and DSS will fill the primary sector first. When the primary sector is full, the secondary sector will be filled by the input from the full cache sector with high IDD. The number of inputs with high EOE and DSS or with high IDD can be changed to alter the data accumulation speed. We use \textbf{selection rate} to represent the ratio of high-ranked text to be selected in cache sector. The cache sector will be emptied once its data fills the primary or secondary sector. 



% % When the secondary sector in any buffers is full, the data in primary sector and secondary sector in every buffer will be extracted and used to fine-tune the LLM. We design \textbf{early stop} strategy to avoid the potential data wasting when the user-generated data concentrating on certain domains. And the personalized LLM can be fine-tuned will less data and learn user-specific data faster.
% When the secondary sector in any buffer is full, the data in the primary and secondary sectors of every buffer will be extracted and used to fine-tune the LLM. We designed an \textbf{early stop} strategy to avoid potential data waste when the user-generated data concentrates on certain domains. Thus, the personalized LLM can be fine-tuned with less data and learn user-specific data faster.

% % As shown in Algorithm ~\ref{alg:on-device_llm}, this logic enables evaluate user input in stream data in a small scale and save storage and computational cost compared with selecting data from a large scale data. 
% As shown in Algorithm ~\ref{alg:on-device_llm}, this logic enables the evaluation of user input in streaming data on a small scale and saves storage and computational costs compared with selecting data on a large scale.


% \subsection{Efficiency of Data Selection}

% Data selection is a process where domain buffers fill the primary and secondary sectors using EDI evaluator. To analyze the efficiency of data selection, we can split the data selection into three parts: (1) complexity of EDI calculation, (2) complexity of retrieval data with high EOE and DSS, and (3) complexity of retrieval data with high IDD. 

% % The proposed EDI evaluator collaborating with domain buffers can effectively select data in terms of spatial and computational efficiency. To analyze the data selection efficiency, 
% \subsubsection{Complexity of EDI Calculation}
% The computational complexity of the EDI calculation involves the tokenization of text, calculation of embedding entropy (EOE), and the domain and semantic score (DSS). Let $N$ be the number of texts, $M$ the average number of tokens per text, and $V$ the size of the vocabulary used in tokenization and embedding.

% \begin{itemize}
%     \item \textbf{Tokenization:} The complexity of tokenizing a text using a pretrained transformer language model tokenizer is $O(M)$.
%     \item \textbf{Entropy of Embedding (EOE):} To compute EOE, we calculate the entropy for each embedding vector. The complexity of this step is $O(M \cdot d)$, where $d$ is the dimensionality of the embeddings.
%     \item \textbf{Domain \& Semantic Score (DSS):} DSS computation involves comparing tokenized text against multiple lexicon dictionaries, resulting in a complexity of $O(M \cdot L)$, where $L$ is the number of lexicons.
% \end{itemize}

% Therefore, the overall complexity for the EDI calculation is $O(N \cdot (M + M \cdot d + M \cdot L)) = O(N \cdot M \cdot (1 + d + L))$.

% \subsubsection{Complexity of Retrieval with High EOE and DSS}
% To retrieve data with high EOE and DSS, we sort texts based on their scores. Assuming the use of an efficient sorting algorithm like heapsort or mergesort:

% \begin{itemize}
%     \item The complexity is $O(N \cdot \log N)$ for sorting based on EOE and DSS scores.
% \end{itemize}

% \subsubsection{Complexity of Retrieval with High IDD}
% The retrieval of data with high IDD involves grouping by dominant domain and then selecting the most distinctive texts within each group:

% \begin{itemize}
%     \item \textbf{Grouping:} The complexity of grouping texts by their dominant domain is $O(N)$.
%     \item \textbf{Selection:} For each domain, selecting the text with the maximum average similarity involves a pairwise comparison within the group. If $g$ is the average group size, the complexity is $O(g^2)$ for each group.
% \end{itemize}

% Given that there are $D$ domains, the total complexity for retrieval with high IDD is $O(N + D \cdot g^2)$.

% Combining these complexities gives us an overall picture of the computational effort required for data selection within the EDI evaluator framework.

% % \subsubsection{Baseline Method Complexity}
% % In the baseline method, where we do not utilize primary and secondary sectors and instead store all data in a single buffer, the computational complexity significantly increases due to the pairwise distinctness computations required for every two pieces of data.

% % Assuming we have $N$ data points and we need to calculate the distinctness between every pair:

% % \begin{itemize}
% %     \item The complexity for computing distinctness between two data points is $O(1)$.
% %     \item To compute the distinctness across all pairs, we perform this computation for each pair, resulting in a complexity of $O(N^2)$, since there are $\frac{N \cdot (N - 1)}{2}$ pairs.
% % \end{itemize}

% % \textit{\textbf{Domain Buffer}}:
% \subsection{Enhance Selected Data by Data Synthesis}

% To effectively fine-tune LLM, semantically similar prompts can increase the model confidence in generating certain expected answers. From this perspective, the large-scaled dataset is necessary due to the high probability to contain such data. However, with significantly limited data, the learning is insufficient for the model to generate certain expected text. To minimize the insufficiency, we propose data synthesis, in which the prompts in selected data are used to generate more similar prompts within a computational acceptable range.

% When the data buffer is full and output the selected data, the deployed LLM, as a generative language model, can be reused as a data generator to diversify the selected prompts. With considering the storage and computational resource constraint, the data synthesis only linearly increase the data size. 


% % \begin{algorithm}
% % \caption{On-Device LLM(input)}
% % \begin{algorithmic}
% % % \STATE Initialize \textbf{Buffers} with domain and data list
% % % \REQUIRE $\textbf{Buffers} \gets \{ 'domain' : \text{data list} \}$
% % % \FUNCTION{onDeviceLLM}{$input$}
% % \STATE { //Domain\_Buffers is a global variable}
% % \STATE $EOE \gets CalculateEOE(input)$
% % \STATE $domain \gets GetDomain(input)$
% % \STATE $DSS \gets CalculateDSS(input)$
% % \STATE $buffer \gets \textbf{Buffers}[domain]$
% % \IF{space in $buffer.primary$}
% %     \STATE $buffer.primary.append((input, EOE, DSS))$
% % \ELSIF{space in $buffer.cache$}
% %     \STATE $buffer.cache.append((input, EOE, DSS))$
% %     \STATE $buffer.primary.append(High\_EOE\_DSS(buffer.cache))$
% %     \STATE $buffer.cache.clear()$
% % \ELSIF{space in $buffer.secondary$}
% %     \STATE $buffer.secondary.append(High\_IDD(buffer.cache))$
% %     \STATE $buffer.cache.clear()$
% % \ENDIF
% % \STATE $SelectedData \gets buffer.primary + buffer.secondary$
% % \IF{$SelectedData$ is not empty}
% %     \STATE $FinetuneLLM(SelectedData)$
% % \ENDIF
% % \end{algorithmic}
% % \end{algorithm}



% % Micro-controller work with IDD.

% % We enable the micro-controller to decide the volume of each dominant domain group. In each group, certain amount of text with the highest DSS will be filled until reach a primary threshold. Then the micro-controller will assign an temporary buffer to each group to hold certain amount of text with high but not higher DDS than the text within the primary threshold. Once the volume of the temporary buffer reach a threshold (secondary threshold), the text with the most dissimilarity compare with the texts within primary threshold will be selected. 
% \subsection{[Need to work on]LLM Personalization Metric}

% % \color{Use ROUGH-1 instead?}
% \textcolor{blue}{Use ROUGH-1 instead?}


% % Evaluate how much the generated text containing relates to the user-specific information is important to LLM for on-device learning. The user-specific information contains the user-LLM interaction history, which can be safely retained in private devices. However, a widely used personalization metric for language model is lacking since it is difficult to contain the conceptual range of personalized information which also leads to the difficulty of quantifying the metric.
% Our framework aims to enhance the LLM capability of causal inference regarding specific users. Different simpler tasks like sequence classification, causal inference cannot be evaluated by prediction accuracy. However, assessing the relevance of generated text to user-specific information is pivotal for on-device learning in LLMs. Such user-specific information encompasses the history of interactions between the user and the LLM, which can be securely stored on private devices. Nonetheless, there is an absence of a universally-accepted personalization metric for language models. This is mainly due to the challenges in capturing the broad spectrum of personalized information, which subsequently makes the metric difficult to quantify.

% % As an alternative, we can measure the generative language model personalization performance via their generated content regarding same prompts. This idea is same as the daily human interaction, where the past and verified answer should be made when people receive the same questions. To quantify the amount of past information the language model can generate, we propose to calculate the cosine similarity of the semantic embedding of the generated content and the original human answers.
% As a solution, we propose assessing the personalization performance of generative language models based on the content they produce in response to identical prompts. This approach mirrors everyday human interactions, wherein individuals are expected to provide consistent and validated answers when posed with the same questions. To quantify the model's ability to reproduce past information, we suggest calculating the cosine similarity between the semantic embeddings of the generated content and the original human responses.

% Given two texts: the original text \( T_o \) and the generated text \( T_g \), we introduce the \textbf{Personalized Correlated Score (PCS)} as:
% \begin{equation}
%     \text{PCS}(T_o, T_g) = \frac{\mathbf{E}_o \cdot \mathbf{E}_g}{\| \mathbf{E}_o \|_2 \cdot \| \mathbf{E}_g \|_2}
% \end{equation}
% % \text{PCS}(T_o, T_g) = \frac{\mathbf{E}_o \cdot \mathbf{E}_g}{\| \mathbf{E}_o \|_2 \cdot \| \mathbf{E}_g \|_2},
% % \]
% where $\mathbf{E}_o$ and $\mathbf{E}_g$ represent the semantic embeddings of \( T_o \) and \( T_g \) respectively, obtained using a pretrained transformer model.


==> table_eval_1.tex <==

% % \begin{table*}
% % \centering
% % \fontsize{6.5}{9.6}\selectfont
% % \caption{Your table caption here}
% % \label{tab:my_label}
% % \begin{tabularx}{\textwidth}{|c|X|X|X|X|X|X|X|X|X|X|}
% % \hline
% %  & Data Size & 0.5\% & 1\% & 2\% & 5\% & 10\% & 15\% & 20\% & 25\% & 30\% \\ 
% % \hline
% % \multirow{5}{*}{\rotatebox{90}{Llama-3B}} &  & & & & & & & & &\\
% %  & & & & & & & & & & \\
% %  & & & & & & & & & &\\
% %  & & & & & & & & & &\\
% %  & & & & & & & & & &\\
% % \hline
% % \end{tabularx}
% % \end{table*}

% % \begin{table*}
% % \centering
% % \fontsize{6.5}{9.6}\selectfont
% % \renewcommand{\arraystretch}{1.5} % Adjusts the height of rows
% % \caption{Evaluate the response quality generated by the LLM finetuned using our proposed framework}
% % \label{tab:my_label}
% % \begin{tabularx}{\textwidth}{|c|X|X|X|X|X|X|X|X|X|X|}
% % \hline
% %  & \textbf{Data Size} & \textbf{0.5\%} & \textbf{1\%} & \textbf{2\%} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{25\%} & \textbf{30\%} \\ 
% % \hline
% % \multirow{5}{*}{\rotatebox{90}{Llama-3B}} & & & & & & & & & & \\
% %  & & & & & & & & & & \\
% %  & & & & & & & & & & \\
% %  & & & & & & & & & & \\
% %  & & & & & & & & & & \\
% % \hline
% % \end{tabularx}
% % \end{table*}

% \begin{table*}
% \centering
% \fontsize{6.5}{9.6}\selectfont
% \renewcommand{\arraystretch}{1.5} % Adjusts the height of rows
% \caption{Evaluate the response quality generated by the LLM finetuned using our proposed framework}
% \label{tab:eval_1}
% \begin{tabularx}{\textwidth}{|c|c|X|X|X|X|X|X|X|X|X|}
% \hline
%  & \textbf{Data Size} & \textbf{0.5\%} & \textbf{1\%} & \textbf{2\%} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{25\%} & \textbf{30\%} \\ 
% \hline
% \multirow{5}{*}{\rotatebox{90}{Llama-3B}} & & & & & & & & & & \\
%  & & & & & & & & & & \\
%  & & & & & & & & & & \\
%  & & & & & & & & & & \\
%  & & & & & & & & & & \\
% \hline
% \end{tabularx}
% \end{table*}


% % \begin{table*}
% % \centering
% % \fontsize{8}{9.6}\selectfont
% % \caption{Your table caption here}
% % \label{tab:my_label}
% % \begin{tabularx}{\textwidth}{|c|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|>{\centering\arraybackslash}X|}
% % \hline
% %  & Data Size & 0.5\% & 1\% & 2\% & 5\% & 10\% & 15\% & 20\% & 25\% & 30\% \\ 
% % \hline
% % \multirow{5}{*}{\rotatebox{90}{Llama-3B}} & ft-domain & & & & & & &  & \\
% %  & &  & & & & & & & \\
% %  & &  & & & & & & & \\
% %  & &  & & & & & & & \\
% %  & &  & & & & & & & \\
% % \hline
% % \end{tabularx}
% % \end{table*}


==> table_eval_2.tex <==
% \begin{table*}
% \centering
% \fontsize{6.5}{9.6}\selectfont
% \renewcommand{\arraystretch}{1.5} % Adjusts the height of rows
% \caption{Evaluate the usage and efficiency of resources}
% \label{tab:eval_2}
% \begin{tabularx}{\textwidth}{|c|c|X|X|X|X|X|X|X|X|X|}
% \hline
%  & \textbf{Data Size} & \textbf{0.5\%} & \textbf{1\%} & \textbf{2\%} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} & \textbf{25\%} & \textbf{30\%} \\ 
% \hline
% \multirow{5}{*}{\rotatebox{90}{Llama-3B}} & Finetune Latency & & & & & & & & & \\
%  & Memory & & & & & & & & & \\
%  & Peak RAM& & & & & & & & & \\
%  & Inference Latency& & & & & & & & & \\
%  & Power Usage& & & & & & & & & \\
% \hline
% \end{tabularx}
% \end{table*}

